Optimal Assistance for Object-Rearrangement Tasks in Augmented Reality

Augmented-reality (AR) glasses that will have access to onboard sensors and an ability to display relevant information to the user present an opportunity to provide user assistance in quotidian tasks. Many such tasks can be characterized as object-rearrangement tasks. We introduce a novel framework for computing and displaying AR assistance that consists of (1) associating an optimal action sequence with the policy of an embodied agent and (2) presenting this sequence to the user as suggestions in the AR system's heads-up display. The embodied agent comprises a "hybrid" between the AR system and the user, with the AR system's observation space (i.e., sensors) and the user's action space (i.e., task-execution actions); its policy is learned by minimizing the task-completion time. In this initial study, we assume that the AR system's observations include the environment's map and localization of the objects and the user. These choices allow us to formalize the problem of computing AR assistance for any object-rearrangement task as a planning problem, specifically as a capacitated vehicle-routing problem. Further, we introduce a novel AR simulator that can enable web-based evaluation of AR-like assistance and associated at-scale data collection via the Habitat simulator for embodied artificial intelligence. Finally, we perform a study that evaluates user response to the proposed form of AR assistance on a specific quotidian object-rearrangement task, house cleaning, using our proposed AR simulator on mechanical turk. In particular, we study the effect of the proposed AR assistance on users' task performance and sense of agency over a range of task difficulties. Our results indicate that providing users with such assistance improves their overall performance and while users report a negative impact to their agency, they may still prefer the proposed assistance to having no assistance at all.

==> Kondo Public/ARsim.tex <==
\section{AR simulator and deployment at-scale}\label{sec:arsimulator}

To evaluate how the proposed AR-assistance model described in Section \ref{sec:arassistance} affects the user experience, an AR simulator must
    (1) support the observations and actions of the embodied-agent policy,
    (2) emulate the first-person view through an AR device, including support of the display of suggestion-notifications in the form of digital objects and information in a heads-up display (HUD), 
    (3) enable a user in the loop to autonomously perform the task-execution actions, and
    (4) be deployable on the web at scale and support data collection related to task performance and sense of agency.

To satisfy the above criteria, we build our AR simulator upon 
Habitat~\cite{savva2019habitat}. 
We make this choice because Habitat satisfies all four of these criteria. First, it supports a suite of embodied-agent observations that mimic the on-board sensors of an AR device (e.g., RGBD video, compass) including those relevant to our current formulation (i.e., mapping and localization of objects and the user). Second, it can display world-locked digital objects and other information that can mimic suggestion notifications in an AR system's HUD, thus supporting the actions of the embodied-agent policy. Third, it supports
3D environments based on real-world reconstructions (e.g., the Replica dataset~\cite{straub2019replica}) rather than synthetically generated environments. Fourth, with modifications, it enables users to perform the task-execution actions required for object-rearrangement tasks. In particular, it natively supports navigation, and we implemented a rudimentary pick/place action as described below. 
%\RD{the new habitat api supports pick and place actions. See: \url{https://colab.research.google.com/github/facebookresearch/habitat-lab/blob/master/examples/tutorials/colabs/Habitat_Interactive_Tasks.ipynb#scrollTo=S426fIt1oDgS}} 
Fifth, Habitat supports the WebGL JavaScript API that enables web-based deployment at scale.
Finally, we note that Habitat supports reinforcement-learning training algorithms (e.g., PPO) \cite{wijmans2019dd} that we can employ to train embodied-agent policies in future studies that assume reduced observation fidelity (e.g., assume only RGBD video); this obviates the need to employ different platforms for policy training and evaluation in future work.


\begin{figure*}[t]
    \centering
    \includegraphics[width=0.7\textwidth]{figs/kondo_ui_v4.pdf}
    \caption{(a)~AR simulator interface with various elements of assistance in the designed virtual HUD.~(b)~Three assistance conditions from the study are shown. Optimal Assistance condition uses both object highlighting via flagpoles and path highlighting via breadcrumbs.}
    \label{fig:assistance_levels}
    \vspace{-0.15in}
\end{figure*}

We make several modifications to Habitat to generate our AR simulator. First, we implement a virtual HUD to mimic the first-person view through an AR device (see Fig.~\ref{fig:assistance_levels}(a)); the HUD supports the display of information relevant to the proposed AR assistance, as well as the ability to display world-locked digital objects in the environment.
A message bar on the top of the HUD alerts users of important interactions, including when the user places an item successfully, or when a user attempts an infeasible action (e.g., attempting to pick/place an item when they are at an excessive distance from a pickup or dropoff location). 
Second, we introduce a `virtual knapsack' of capacity two that represents the user's current inventory; we display the current contents of this backpack as the user's inventory in the virtual HUD.
Third, we introduce a rudimentary object pick/place action that either (1) picks up an object and places it in the virtual knapsack if the user is within a specified distance of a pickup location and the knapsack is not full, or (2) places an object in inventory in its dropoff location if the user is within a specified distance of the dropoff location and the associated object is in inventory. Fourth, we integrate Habitat with the OR-Tools planner to support real-time replanning as described in Section \ref{sec:CVRP}.


By leveraging Habitat's existing WebGL JavaScript API, we can deploy our AR simulator at scale on AMT and collect data related to task performance and sense of agency by leveraging psiTurk \cite{gureckis2016psiturk}. Appendix \ref{sec:system_implementation} describes the details of this setup. 

% \KTC{Use the same arguments from the intro: (1) support of 3D environments based on real-world reconstructions rather than synthetically generated environments, (2) support of embodied-agent observations that mimic the on-board sensors of an AR device (e.g., RGBD video, compass, localization, mapping, object tracking), (3) support of the task-execution actions required for object-rearrangement tasks (i.e., navigation, picking up and placing objects), (4) ability to display world-locked digital objects and other information that can mimic suggestion notifications in an AR system's heads-up display, and (5) support of the WebGL JavaScript API that enables web-based deployment at scale using, e.g., Amazon Mechanical Turk (AMT)}

% 1. Challenge of collecting human data at scale. 
% i. Where we fit on spectrum low-fidelty/high-scale to high-fidelty/low-scale.
% ii. Understanding how this framework can be used to approach high-fidelity or be used in conjunction with high-fidelity/low-scale experiment. 
% Show results from the survey responses on realism use in real world 

==> Kondo Public/assistance.tex <==
\section{AR-Assistance Model}\label{sec:arassistance}

The goal of our AR assistance model is to formalize the problem of computing and displaying AR assistance for object-rearrangement tasks.  We achieve this by adopting the perspetive of embodied AI and (1) associate an optimal action sequence with the policy of an embodied agent, and (2) present this optimal action sequence to the user as suggestion notifications in the AR system's heads-up display. To particularize this setup, we must define the embodied agent and associated partially observable Markov decision process (POMDP) ingredients: the states, observations, actions, and rewards characterizing the environment, agent, and task.

\subsection{Embodied AI formulation}

We begin by defining the objective (and associated reward) of the task as moving each object in question from its initial position to its final desired position in as little time as possible. Minimal time to task completion is not only an intuitive choice for an objective and reward, it also draws inspiration from the long history of AI assistants for task and time management~\cite{myers2007intelligent}.

Regarding the choice of embodied agent, one could adopt a fully multiagent perspective and 
consider the user and AR system to be independent but cooperating agents with the shared aforementioned objective but with different observation and action spaces. In this case, one could learn the AR system's policy and present its action sequence to the user as suggestion notifications. Unfortunately, this approach introduces significant challenges, as the user is included in the AR system's environment and thus any simulation-based learning algorithm for the AR-system's policy would require modeling the user's policy acting on an observation space augmented by the AR-system's displayed information \cite{bucsoniu2010multi}. Instead, we simplify this setup and consider a single-agent formulation with an agent comprising a `hybrid' between the AR system and the user. Namely, it has the observation space (i.e., sensor measurements) of the AR system and the actions (i.e., physical task-execution actions) of the user; in the case of object-rearrangement tasks, the latter corresponds to navigation and object pick/place actions. In this case, learning- or planning-based approaches for computing the embodied agent's policy require modeling only the physical dynamics of object rearrangement.

As mentioned above, the embodied-agent's observations correspond to those of the AR system. While many current AR head-mounted devices are equipped with only RGB video, future devices are likely to be equipped with much more high-fidelity observations. Indeed, it is likely that---at least for familiar environments---the AR device will have access to a complete map and will be able to perform localization of the user and objects \cite{livemaps}. As such, for this initial study, we assume that the AR device can has complete observations that include a map of the environment, the current position of all objects in question, and the position of the user. Thus, the observations and state coincide in this case, and the POMDP reduces to an MDP with deterministic transition dynamics, exposing the use for a deterministic planner as described in Sec.\ \ref{sec:CVRP}.

Finally, we assume that the user can carry only two objects at once, the AR device has knowledge of the desired final location of all objects in question (i.e., the `goal state' of the environment), and the AR device can calculate the shortest path between any two points on the map. These assumptions allow us to compute the policy of the embodied agent by a planner that solves a capacitated vehicle routing problem (CVRP), which we describe in Sec.\ \ref{sec:CVRP} below.
We remark that future work will relax the above assumptions and consider multiagent formulations, partial observations, and model-free learning of embodied-agent policies.

\subsection{Object-rearrangement planner: capacitated vehicle routing problem}\label{sec:CVRP}

We now formulate the (single-vehicle) CVRP \cite{dantzig1959truck,golden2008vehicle} for object-rearrangement tasks. We assume that we are rearranging $\nobjects$ objects such that each object has an initial location and final (desired) location, thus yielding $2\nobjects+1$ total locations of interest (including the initial position of the user). Given any arbitrary enumeration of these locations with the zeroth location corresponding to the user's initial position (i.e., the \textit{depot}), we decompose these locations into \textit{pickup locations} $\objectLocations\subset\natno{2\nobjects}$ associating with the objects' current locations and \textit{dropoff locations} $\receptacleLocations\subset\natno{2\nobjects}$ associated with the final locations such that $|\objectLocations| = |\receptacleLocations| = \nobjects$, $\objectLocations\cap\receptacleLocations = \emptyset$, and $\objectLocations\cup\receptacleLocations = \natno{2\nobjects}$. We assume that \textit{transportation costs} can be calculated from an operator $\distanceNo:\natnoZero{2\nobjects}\times \natnoZero{2\nobjects}\rightarrow\RRplus{}$ that calculates the geodesic distance between any two locations and satisfies $\distance{i}{i} = 0$, $i\in\natnoZero{2\nobjects}$. If any two pickup or dropoff locations $i$ and $j$ coincide, we treat them as separate locations with zero separating distance such that $\distance{i}{j}=0$. 
This assumes the user's time to complete the task is proportional to their total path length.
We assume the user has a \textit{capacity constraint} of $\capacity\in\mathbb N$ (which we set to be $\capacity = 2$ in the experiments, which assumes a user can carry one object per hand). We introduce a delivery operator $\receptacleNo:\objectLocations\rightarrow\receptacleLocations$ that maps each pickup location to its corresponding dropoff location. We associate any solution to the problem with an invertible operator $\stepToLocNo:\natnoZero{2\nobjects}\rightarrow\natnoZero{2\nobjects}$ that maps the step number to location index; note that invertibility of this operator assumes that each location is visited exactly once and a location visit is associated with the pickup or dropoff of the appropriate object. Assuming the user has already executed $m(\leq 2\nobjects)$ steps of the task by visiting locations $\stepToLocTaken{0},\ldots,\stepToLocTaken{m}$ with $\stepToLocTaken{0}=0$ and the task initialized at $m=0$, the planner defines the optimal sequence of location visits $(\stepToLocOpt{0},\ldots,\stepToLocOpt{2\nobjects})$ as the solution to the combinatorial optimization problem
\begin{align}\label{eq:CVRP}
\begin{split}
\underset{(\stepToLoc{0},\ldots,\stepToLoc{2\nobjects})}{\text{minimize}}\ &\sum_{i=1}^{2\nobjects}\distance{\stepToLoc{i}}{\stepToLoc{i-1}}\\
\text{subject to}\ &\sum_{i=1}^j\indicatorFunctionTwo{\objectLocations}{\stepToLoc{i}} - \indicatorFunctionTwo{\receptacleLocations}{\stepToLoc{i}}\leq\capacity,\quad \forall j\in\natno{2\nobjects}\\
&\locToStep{\receptacle{i}} > \locToStep{i},\quad \forall i\in\objectLocations\\
& \stepToLoc{i} = \stepToLocTaken{i},\quad \forall i\in\natnoZero{m},
\end{split}
\end{align}
where $\indicatorFunction{A}$ is the indicator function that evaluates to 1 if its argument is in the set $A$ and evaluates to zero otherwise.

The objective function in problem \eqref{eq:CVRP} corresponds to the transportation costs (i.e., total distance traveled); the first set of constraints corresponds to the capacity constraints; the second set of constraints ensures that each object's pickup location is visited before its dropoff location; the third set of constraints enforces that the solution is computed from the current state of the task at step $m$. Given the solution $(\stepToLocOpt{0},\ldots,\stepToLocOpt{2\nobjects})$ to problem \eqref{eq:CVRP}, at step $p(\geq m)$ of the task, the AR device provides assistance by displaying to the user the shortest path between locations $\stepToLocOpt{p}(=\stepToLocTaken{p})$ and $\stepToLocOpt{p+1}$ in the form of world-locked digital breadcrumbs in the heads-up display. If the user `violates' assistance and instead visits a feasible alternative location $\stepToLocTaken{p+1}(\neq\stepToLocOpt{p+1})$, then the system replans by solving problem \eqref{eq:CVRP} with $m\leftarrow p+1$ and resumes. We emphasize that replanning is essential to ensure robustness to realistic user behavior in complex multi-step object-rearrangement tasks.
In practice, we solve planning problem \eqref{eq:CVRP} using OR-Tools \cite{OR-Tools}.

%
%This formulation implicitly assumes that the user will directly follow any 
%
%
%complex dynamics between the user and AR device, as well as the user's own suboptimal policy , rather than With this view, we can consider the observations of the user to comprise all the sensory signals of the central nervous system, and the action space corresponding to the task-execution actions of navigation, object picking, and object placing.




% It is unclear how should one design assistance strategies for AR that could lead to improved quality of life for its users~\cite{}. Central to our work is the hypothesis that assistance that leads to reduced effort or time to completion in a task would be of value to the user. We are inspired by the long history of AI-powered assistants for task and time management~\cite{myers2007intelligent}. 

% Our focus is on every-day tasks that involve multiple steps. Assisting users with such tasks requires the understanding of the task that the user is aiming to do or in other words, the goal/intent of the user. However, instead of estimating user's intent and the desired task by observing user actions~\cite{fern2007decision}, we assume that the user's task is known apriori. This also follows the conventional interaction style of invoking conversational assistants such as Siri, where the user prescribes their intended task clearly. In the future, we hope to relax this assumption and compute assistance based on inferred user-goals by leveraging approaches such as Inverse Reinforcement Learning~\cite{jara2019theory}.


%\subsection{Overview}
%The problem of finding optimal sequence of actions for a task is well-studied within the fields of Reinforcement Learning (RL) and Planning~\cite{sutton2018reinforcement}. Typically, the actions are associated with a learning agent who learns to map the current state and context in the task to an action such that a task-specific goal is achieved~\cite{sutton2018reinforcement}. The function that maps a state to an action given a goal, also known as a policy, is usually computed by solving an optimization problem. This approach of computing optimal actions (policy) is fairly generic and applies to a broad category of problems. For instance, in a self-driving scenario, the agent

%In the house-cleaning scenario, the actions could correspond to navigating to various objects and picking and placing them, while the state could correspond to the current location of the user and the positioning of all the objects in the house.

%\subsection{User + AR `super agent'}

%\subsection{Task}

==> Kondo Public/commands.tex <==
\usepackage{amsmath,amsfonts}
\newcommand{\nobjects}{n}
\newcommand{\capacity}{c}
\newcommand{\stepToLocNo}{x}
\newcommand{\stepToLocOptNo}{\stepToLocNo^\star}
\newcommand{\stepToLocTakenNo}{\bar\stepToLocNo}
\newcommand{\stepToLoc}[1]{\stepToLocNo(#1)}
\newcommand{\stepToLocOpt}[1]{\stepToLocOptNo(#1)}
\newcommand{\stepToLocTaken}[1]{\stepToLocTakenNo(#1)}
\newcommand{\locToStep}[1]{\stepToLocNo^{-1}(#1)}
\newcommand{\natno}[1]{\{1,\ldots,#1\}}
\newcommand{\natnoZero}[1]{\{0,\ldots,#1\}}
\newcommand{\objectLocations}{\mathcal P}
\newcommand{\receptacleLocations}{\mathcal D}
\newcommand{\indicatorFunction}[1]{{\boldsymbol 1}_{#1}}
\newcommand{\indicatorFunctionTwo}[2]{\indicatorFunction{#1}(#2)}
\newcommand{\distanceNo}{d}
\newcommand{\distance}[2]{\distanceNo(#1,#2)}
\newcommand{\receptacleNo}{f}
\newcommand{\receptacle}[1]{\receptacleNo(#1)}
\newcommand{\RR}[1]{\mathbb R^{#1}}
\newcommand{\RRplus}[1]{\mathbb R_+^{#1}}
\usepackage{titlesec}
\titlespacing*{\section}{0pt}{0.3\baselineskip}{0.3\baselineskip}
\titlespacing*{\subsection}{0pt}{0.1\baselineskip}{0.1\baselineskip}

==> Kondo Public/discussion.tex <==
\section{Conclusions}

This work has presented (1) a novel framework for computing and displaying AR assistance for object-rearrangement tasks that characterize a broad category of quotidian tasks, (2) a novel AR simulator that can enable web-based evaluation of AR-like assistance and large-scale data collection, and (3) a study that assesses how users respond to the proposed AR assistance in the AR simulator on a specific object-rearrangement task: house cleaning.

The study illustrated several salient trends. First, by following the optimal assistance, participants were able to reduce the overall distance they travelled, suggesting that people do not immediately solve this problem optimally and could benefit from a system like the one we propose. Second, though participants' reported feeling less in control over their own actions when following the optimal assistance they were also more likely to agree that they preferred a system that told them what to do than users in either other group. This indicates that users may be willing to sacrifice a small amount of agency in favor of a system that provides useful assistance. Finally, users were less likely or equally likely to accept the assistance as the difficulty of the task increased, though the population of users in the optimal assistance condition exhibited a much wider variability of assistance acceptance. This indicates that there are potential subgroups in the user population, and that future work should be conducted to discover these groups and develop personalized assistance systems.  

Future work will explore extensions of the current framework and study, including developing and assessing perception-based learned policies that assume lower fidelity of the embodied agent’s observations, considering multi-agent formulations that incorporate models of the user’s behavior, and extending the current assistance framework and AR simulator to other quotidian object-rearrangement tasks and assessing the user experience in those settings.











% \subsection{Completion Time}
% Participants who saw  task difficulty level zero completed the  task significantly faster than those  in other groups. Interestingly, participants in tasks difficulties 1 through 4 did not complete the task in significantly different times, indicating that either people were having a good time with the task and wanted to continue to interact with the environment, or that task difficulty does  not vary smoothly as we implicitly thought by varying the task difficulties in the way we did. Additionally, while participants in who saw the optimal assistance in task difficulty 0 did complete the task faster than in the other two groups, this different was not found to be significant. Another interesting observation is how wide the error bars are, indicating the wide range of human performance on this task, at least with respect to time. To develop assistance algorithms that can be effective at decreasing a user's time to complete the chore, more personalized or individual studies may be beneficial.  

% \subsection{Performance Against Optimal}

% \subsubsection{Distance}
% Comparing participant path distances to the optimal path distances showed that users who saw the optimal assistance condition achieved path lengths more similar to the optimal path length than those who saw no assistance. In fact, on average, participants who saw the optimal assistance score approximately 8 points higher on the IPL metric than those who saw no assistance. The majority of this boost seems to be coming from the easiest task difficulty though. This is interesting, as  it suggests users are less likely to follow the breadcrumb trails as the task gets more difficulty, even though they were told that there objective was to minimize the time they spent in the task and that these paths would help them achieve this goal.

% \subsubsection{Ordering}
% Participants who saw the optimal assistance condition were approximately $25\%$ less likely to deviate from the ordering suggested to them by the assistance system, but this was not constant across difficulty conditions. As the task became more difficult, users were more likely to deviate from the optimal ordering. This  suggests that as the task becomes more difficult, users are increasingly less likely to follow the optimal path, even though this would minimize their time spent in the task. Additionally, the error bars on the optimal assistance condition are much larger than the other assistance conditions, suggesting that there are different groups within the optimal assistance condition (\textit{e.g.} those who listen to the optimal ordering, and those who do not). 


% Future work buckets:
% 1. multi-agent


% % - as a data collection framework for:
% % -- ar user experiments
% % -- human performance evaluation datasets

% % - developing more ar assistance models



==> Kondo Public/related.tex <==
\section{Related Work}
We now review related work that relates to our three key contributions. Namely, we review existing work in AR assistance in Sec.\ \ref{sec:ARassistance}, simulation frameworks for training and evaluating embodied-agent policies in Sec.\ \ref{sec:simulationFrameworks}, and assessing users' response to digital assistance in Sec.\ \ref{sec:usersresponse}.

\subsection{AR assistance}\label{sec:ARassistance}

To date, most work on employing AR devices to assist users has focused on displaying \textit{predefined information overlays} that can be useful in 
completing a prescribed task; the information overlays are often spatially registered to objects or locations relevant to the task. For example, researchers have investigated approaches wherein the AR device overlays information or instructions on parts to be assembled or maintained \cite{thomas1992augmented,tang2003comparative}, retrieves and displays maintenance documentation using object recognition \cite{didier2005amra},  overlaying medical imaging data on patients in real time \cite{bajura1992merging}, or provides location and activity-based, world-locked information to the users during indoor navigation~\cite{mulloni2011handheld}.

Critically, none of the above approaches are truly robust for complex multi-step tasks, as they do not leverage the device's on-board sensors to infer the current task state; as such, they are unable to provide the user with up-to-date assistance toward optimal task completion or properly adapt when users deviate from the system's suggested steps. To fill this gap, planning-based\footnote{Planning refers to the process of computing an agent's policy using a model for the transition dynamics of the environment, i.e., a model that predicts the effect of the agent's actions on the environment states~\cite{sutton2018reinforcement}.} approaches that track task state in real time and update assistance accordingly have been proposed for a variety of AR applications such as robot tele-operation~\cite{tzafestas2001teleplanning, fang2014novel}, assistive surgery~\cite{bourquain2002hepavision2}, assembly and manufacturing~\cite{abramovici2017context}, and even an quotidian task of sandwich assembly~\cite{hu2020interactive}. In particular, Abramovici et al.~\cite{abramovici2017context} enable AR assistance for collaborative manufacturing using a complex back-end infrastructure where smart devices broadcast their status to a centralized planner with a predefined task dependency graph. 

Instead, our proposed approach for AR assistance applicable to complex object-rearrangement tasks described in Sec.\ \ref{sec:arassistance} leverages only the sensor measurements of the AR device, and executes a policy whose state is informed only by these sensor measurements, thus enabling up-to-date assistance toward optimal task completion. In this initial study, we assume the device has `full environment knowledge' via its sensors and can support mapping and localization of the user and objects \cite{livemaps}. This allows us to compute the policy using a planner based on a capacitated vehicle routing problem. Perhaps the most closely related work to ours is the planning-based cognitive assistant developed by Hu et al.~\cite{hu2020interactive}, which employs a perception module driven by computer vision to identify task state in a sandwich-assembly task and re-plan using a finite state machine. 
In contrast to this work, we consider a much broader category of object-rearrangement tasks and consider planners based on a general capacitated vehicle routing problem as described in Sec.~\ref{sec:CVRP}. Further, our embodied AI formulation enables straightforward extensions that go beyond the strict environment-knowledge requirements of planning to learning policies that can employ perception-based partial environment observations.

 \subsection{Embodied-agent simulation frameworks}\label{sec:simulationFrameworks}
% TLDR: our use of simulation is unique: to emulate AR experience and to evaluate at scale
The robotics and embodied AI communities have leveraged simulation frameworks to train and evaluate embodied-agent policies in lieu of expensive real-world experimentation infrastructure ~\cite{savva2019habitat, ai2thor, koenig2004design, erickson2019assistive}. Most efforts consider fully autonomous agents (e.g. robots) whose actions directly change the physical state of the environment. 

Our AR-assistance application is fundamentally different from these, in that actions that can modify the physical state of the environment belong to the human agent. The AR device (our parallel to the autonomous system) can only influence the physical state of the environment indirectly via suggestion-notification actions displayed to the human. Thus, for AR assistance, any realistic \textit{evaluation} of the how the embodied-agent policy affects task performance must involve a human in the loop---or a high-fidelity model of the human's behavior. Evaluating how assistance affects important qualitative aspects of the user experience (e.g., effort, sense of agency) necessitates collecting data from real users at scale. On the other hand, \textit{training} of the embodied-agent policy can be done in a variety of ways that need not rely on a human in the loop; Sec.\ \ref{sec:arassistance} describes in detail our proposed formulation for computing the policy that does not require a human in the loop---only a planner coupled to a simulator that can compute the geodesic distances between locations and track task state---although future work will consider human-in-the-loop training loop analogously to Refs.~\cite{li2016dialogue, zhang2019leveraging}. Thus, for learning assistive AR policies, rather different demands are placed on the environments used for \textit{evaluation} and \textit{training}; the only strong compatibility requirement is that the evaluation environment must support the states and actions associated with the trained policy to deploy it in real time. Here, we focus on the evaluation environment.

Arguably the closest related work is in the field of human--robot interaction (HRI), where researchers are interested in evaluating users' response to robotic assistance~\cite{brooks2018brave}. In this field, the two most common evaluation environments comprise either (1) in-person studies where users are asked to respond to robotic assistance~\cite{dragan2013legibility}, and (2) web-based studies where users are asked to view third-person videos or photos of humans and robots interacting and react accordingly~\cite{hoffman2019evaluating, malle2016robot}. The former category suffers from lack of scalability, while the latter category lacks immersion due to its reliance on a third-person perspective. 

Thus, we believe that our proposed evaluation framework---which is based on an AR simulator and is described in Sec.\ \ref{sec:arsimulator}---combines the attractive attributes of each of these paradigms, as it enables scalable, first-person interaction of a user with an embodied assistant and thus we hypothesize can capture more realistic user experiences---and thus yield higher quality user-experience data---at scale. 

\subsection{Evaluating user response to digital assistance}\label{sec:usersresponse}
It is generally challenging to characterize the user experience for digital assistance owing to a plethora of factors involved and owing to the difficulty of measuring some of these factors with high fidelity~\cite{albert2013measuring}. Past studies on evaluating users' response to digital assistance have focused on evaluating factors such as usability, utility, effectiveness, and agency~\cite{berry2009evaluating}. 
In our study, we focus primarily on evaluating effectiveness as measured by the user's task performance and sense of agency. We focus on task performance as it is easy to measure and directly addresses the key value proposition of AR assistance for complex tasks. We consider agency due to its central role in human--computer interaction (HCI) research and its relatively uncharacterized role in immersive AR-like assistive scenarios.

The sense of agency refers to the feeling of being in the driver's seat when it comes to selecting one's actions~\cite{moore2016sense}. HCI research has long recognized the sense of agency as a key factor in characterizing how people experience interactions with technology~\cite{limerick2014experience,moore2016sense, shneiderman2010designing}. In particular, one of the eight classic rules of interface design places emphasis on designing interfaces that support the user's sense of agency~\cite{shneiderman2010designing}. Further, the sense of agency may also influence a user's acceptance of technology~\cite{baronas1988restoring, le2018agency}. Despite the importance of agency, it has received limited attention in the domain of AR. It is important to address this topic early in developing novel AR technologies, as enabling user's sense of agency is indeed challenging in assistive and immersive systems; for example, previous research has found a reduction in sense of agency with increase in automation~\cite{berberian2012automation}. 

The study presented in Sec.\ \ref{sec:study} evaluates task performance and the user's sense of agency on the proposed cleaning-house task.
Akin to other studies on AR assistance that have shown improved task performance for instance in assembly tasks~\cite{yang2019influences, tang2003comparative}, we show faster task completion times with the use of the proposed AR assistance. Further, we study the effectiveness over a range of task-difficulty and assistance-fidelity levels. 
Our study also suggests that while reports of user agency may be negatively affected by increased assistance in this scenario, this may be a cost participants are willing to pay in order to realize improved task performance; these are promising results, and can serve as a baseline for alternative interfaces for displaying the computed AR assistance to the user.



% Key criteria: task performance, effort, and sense of agency.
% \begin{itemize}
%     \item See this paper on "assessing effectiveness of AR instructions in an assembly task" \cite{tang2003comparative}. They assess "task performance
% and perceived mental workload".
% \end{itemize}
% TL;DR: Limited knowledge about how users respond to assistance that manipulates their sense of physical environment directly.


==> Kondo Public/results.tex <==
\section{User study}

We conducted a $3\times 4$ between-subjects user study ($n=447$ participants, male$=265$, female$=177$, other$=1$, no answer$=4$; three assistance-fidelity levels; four task-difficulty levels) on AMT using our AR simulator setup described in Sec.~\ref{sec:arsimulator}. Participants were compensated $\$7.50$ for completing the 25-minute-long study. Appendix~\ref{sec:studyparticipants} reports details on the number of participants in each condition. We first present and evaluate the hypotheses related to different assistance fidelity in easiest task difficulty condition using objective and subjective metrics defined in Sec.~\ref{sec:study}. We then show the interaction effects between assistance and task difficulty.  

\subsection{Effects of varying assistance fidelity}\label{sec:assistance}
We now conduct a study that varies the assistance fidelity and fixes task difficulty to the easiest level (i.e., 6 total objects).

\subsubsection{Hypotheses.}
With regards to varying the assistance fidelity, we had the following hypotheses:
\begin{itemize}
    \item[\textbf{H1}] Participants will follow optimal assistance when presented with it.
    \item[\textbf{H2}] Participants will have higher task performance when presented with optimal assistance.
    % \item[\textbf{H3}] Participants will be more likely to respond that they are adhering to optimal assistance than to no assistance or object-highlighting assistance. 
    \item[\textbf{H3}] Participant agency will be unaffected by assistance fidelity. 
    \item[\textbf{H4}] Participants will perceive the AR system equipped with optimal assistance as more usable and useful than the AR system equipped with no assistance or object-highlighting assistance.
\end{itemize}

\subsubsection{Results summary} We now present results for the varying-assistance-fidelity study in terms of both objective and subjective metrics. For an in-depth reporting of the statistical analyses, see Sec.~\ref{sec:statAssistance} and Figs.~\ref{fig:easy_deviations}--\ref{fig:easy_distance}.

\begin{figure}[t]
    \centering
    \begin{minipage}[t]{.31\linewidth}
        \includegraphics[width=\linewidth]{figs/easy_deviations.pdf}
        \caption{On average participants in the optimal condition deviated from the optimal ordering less frequently than participants in object-highlighting ($p<0.001$) and no assistance conditions ($p<0.001$).}\label{fig:easy_deviations}
    \end{minipage}\hfill
    \begin{minipage}[t]{.31\linewidth}%
        \includegraphics[width=\linewidth]{figs/easy_ipl_end.pdf}
        \caption{Participants provided with optimal assistance followed paths that more closely resembled the optimal paths than in object-highlighting ($p<0.01$) and no assistance conditions ($p<0.001$).}\label{fig:easy_ipl}
    \end{minipage}\hfill
    \begin{minipage}[t]{.31\linewidth}%
        \includegraphics[width=\linewidth]{figs/easy_distance.pdf}
        \caption{Participants provided with optimal assistance ($p<0.001$) and object-highlighting assistance ($p<0.01$) were more likely to find shorter paths than participants in the no assistance condition.}\label{fig:easy_distance}
    \end{minipage}
    \vspace{-0.15in}
\end{figure}

\textbf{Objective metrics}. In the case of optimal assistance, we observe that participants are more likely to pick and place items in the optimal order than they are in either the none or object-highlighting assistance conditions as measured by normalized deviations (Fig.~\ref{fig:easy_deviations}). \emph{This suggests that people may not able to compute independently the optimal ordering of location visits for object-rearrangement tasks based on only a first-person perspective, even with object highlighting}. Further, in the case of optimal assistance, participants follow the shortest-path trajectory between points more closely than they do in either the no assistance or object-highlighting assistance conditions (see IPL in Fig.~\ref{fig:easy_ipl}). \emph{This suggests that when participants freely navigate within an environment, they do not naturally take the shortest paths to get from point to point.} Taken together, these two findings support our hypothesis H1 that participants will follow optimal assistance when presented with it.

Even though participants tend to follow optimal assistance, this does not necessarily translate to improvements in all performance metrics. We measure task performance in two additional ways: total distance traveled and total task completion time. We observe that participants presented with object-highlighting and optimal assistance generated significantly shorter total paths than those generated in the no-assistance case, but the average path length traveled with these two forms of assistance was not substantially different (Fig.~\ref{fig:easy_distance}). \emph{This indicates that it is possible to get users to follow shorter paths than those they might find on their own, but that simply highlighting objects may be sufficient for decreasing user path distance. Interestingly, even though participants found shorter paths in the optimal and object-highlighting conditions, there was no significant difference in the total task completion time between the three conditions.} This further indicates that even though we are able to shorten path length, this may come at some cost to the speed at which a user completes the task (potentially in the interpretation of the interface). Ultimately, navigating this trade-off is likely user or task specific, and can likely be made more favorable with alternative and personalized interface design. Taken together, these two findings partially confirm our hypothesis H2 that participants will have higher task performance when presented with optimal assistance. 

\textbf{Subjective metrics}. \textit{Agency.} We found that participants generally felt in control of what they should do next and how quickly they completed the task. Even so, participants provided with optimal assistance, while still generally agreeing with feeling in control, reported that they felt less in control than in the other assistance conditions. Participants provided with no assistance and object-highlighting assistance were neutral about their feelings of needing to follow the assistance; participants provided with optimal assistance rated that they did feel the need to follow the assistance. Finally, participants provided with no assistance and object-highlighting assistance disagreed that they would prefer to have the system show them what to do next and where to go next. Since they were not exposed to a condition where they were provided this information, they are likely rating this against their idea of what such a system might look like. \emph{Participants who actually were exposed to optimal assistance agreed that they preferred this to not having this assistive information. So, even though participants in the optimal assistance condition felt less in control overall, they seemed to prefer this than to an alternative}. Overall, this does not support our hypothesis H3 that participants' sense of agency would remain unaffected by assistance fidelity; however, it seems that despite feeling a slight loss in their sense of agency, they may actually prefer this sacrifice in order to obtain useful information for optimal task completion.

\textit{Usability and Utility}. We found that participants generally felt that they were faster with assistance than without assistance. \emph{Participants provided with both optimal assistance and object-highlighting assistance believed that they completed the task faster with the additional information than they would have without it (i.e., with no assistance).} While participants in all assistance-fidelity conditions perceived the assistance to be useful, \emph{those provided with optimal assistance perceived it to be more useful than in either the object-highlighting or no assistance conditions.} These results are especially interesting given that no significant difference was found in total task completion time between assistance-fidelity levels. Overall, these findings partially support our hypothesis H4 that participants will be more likely to perceive the optimal assistance to be usable and useful than other assistance types. 

% \begin{figure}[t]
%     \centering
%     \begin{minipage}[t]{.31\linewidth}
%         \includegraphics[width=\linewidth]{figs/easy_deviations.pdf}
%         \caption{On average participants in the optimal condition deviated from the optimal ordering less frequently than participants in object-highlighting ($p<0.001$) and no assistance conditions ($p<0.001$).}\label{fig:easy_deviations}
%     \end{minipage}\hfill
%     \begin{minipage}[t]{.31\linewidth}%
%         \includegraphics[width=\linewidth]{figs/easy_ipl_end.pdf}
%         \caption{Participants provided with optimal assistance followed paths that more closely resembled the optimal paths than in object-highlighting ($p<0.01$) and no assistance conditions ($p<0.001$).}\label{fig:easy_ipl}
%     \end{minipage}\hfill
%     \begin{minipage}[t]{.31\linewidth}%
%         \includegraphics[width=\linewidth]{figs/easy_distance.pdf}
%         \caption{Participants provided with optimal assistance ($p<0.001$) and object-highlighting assistance ($p<0.01$) were more likely to find shorter paths than participants in the no assistance condition.}\label{fig:easy_distance}
%     \end{minipage}
% \end{figure}



\begin{figure}[t]
    \centering
    \includegraphics[width=.75\linewidth]{figs/monster.png}
        \caption{\textbf{Left}, When compared against no assistance and object-highlighting assistance, participants in the optimal assistance condition were less likely to feel in control (both $p<0.001$), more likely to feel the need to follow the assistance (both $p<0.01$), and more likely to prefer being told what to do (both $p<0.001$). \textbf{Right}, Participants in the optimal assistance were more likely to rate assistance as usable ($p<0.001$) and useful than those provided with no-assistance ($p<0.001$).  Those in object-highlighting more strongly agreed that the assistance was useful when compared to no-assistance ($p<0.05$). Those in optimal assistance more strongly agreed that the assistance was useful as compared to the object-highlighting assistance ($p<0.05$). }\label{fig:easy_monster}
   \vspace{-0.15in}
\end{figure}

\subsection{Interactions between assistance and task difficulty}\label{sec:interactions}

\subsubsection{Hypothesis.}
We had the following hypothesis:
\begin{itemize}
    \item[\textbf{H5}] As the task difficulty increases, participants will be more willing to accept the assistance.
\end{itemize}

\subsubsection{Results summary.}
For an in-depth reporting of the statistical analyses, see Sec.~\ref{sec:statInteraction} and Fig.~\ref{fig:int_ipl}.

Across the board, we observed that participants deviated more from the optimal ordering as task-difficulty increased (Fig.~\ref{fig:int_ipl}). In the cases of no assistance and object-highlighting assistance, this trend conforms to our expectation that people have difficulties in finding the optimal solution in object-rearrangement tasks. We still observe this trend, however, when people are explicitly given the optimal ordering as in the optimal-assistance condition. Interestingly, though, the variance in the optimal-assistance condition is consistently much greater than those in either the no assistance or object-highlighting assistance cases. This suggests that the underlying distribution of assistance acceptance is likely multi-modal, and future work can investigate mechanisms to increase acceptance among various sub-populations of users. 

\emph{We also observed that participants were more likely to take shorter paths in the optimal-assistance condition than in the other two conditions, and that participants provided with object-highlighting assistance were more likely to take shorter paths than those provided with no assistance (Fig.~\ref{fig:int_ipl})}. However, there was no change in IPL as the task-difficulty level increased. Taken together, this refutes our hypothesis H5 that users would be more likely to accept assistance as the task became harder. In fact, the data suggest that they are either less likely or just as likely to accept the assistance as the task difficulty increases. 

\begin{figure}[t]
    \centering
    \begin{minipage}[t]{.06\linewidth}%
    \end{minipage}\hfill
    \begin{minipage}[t]{.4\linewidth}
        \includegraphics[width=\linewidth]{figs/int_deviations.pdf}
        
    \end{minipage}\hfill
    \begin{minipage}[t]{.06\linewidth}%
    \end{minipage}\hfill
    \begin{minipage}[t]{.4\linewidth}%
        \includegraphics[width=\linewidth]{figs/int_ipl.pdf}
      
    \end{minipage}\hfill
        \begin{minipage}[t]{.06\linewidth}%
    \end{minipage}\hfill
    \caption{\textbf{Left}, participants provided with optimal assistance were less likely to deviate from the optimal ordering than participants provided with either no assistance or object-highlighting assistance ($p<0.001$, both). As the difficulty increased, participants were more likely to deviate in each group. \textbf{Right}, participants provided with optimal assistance were more likely to follow shortest paths (higher IPL) than those provided with both object-highlighting ($p<0.01$) and no ($p<0.001$) assistance. Participants provided with object-highlighting assistance took shorter paths than those in none ($p<0.001$).}  \label{fig:int_ipl}
    \vspace{-0.15in}
\end{figure}



==> Kondo Public/study.tex <==
\section{Study setup}\label{sec:study}

The overarching goal of our study is to evaluate
how users respond to the AR assistance generated by the proposed framework on a specific quotidian object-rearrangement task---house cleaning---using our proposed AR simulator. Sec.\ \ref{sec:task} describes the house-cleaning task. Sec.\ \ref{sec:studyConditions} describes the two key variables that we varied during the study. Sec.\ \ref{sec:metrics} describes the metrics that we employed to evaluate the user experience. Sec.\ \ref{sec:hitoverview} provides an overview of the Human Intelligence Task (HIT) characterizing our study.

\subsection{House-cleaning task}\label{sec:task}
The main house-cleaning task is explained to participants through the following prompt: 
\begin{quote}
In this HIT, you are a guest at a short-term rental. You have been staying at the house for the past several days and checkout time is fast approaching. You must clean up this house according to the host’s instructions in as little time as possible. In order to avoid a late fee, you must navigate through the house to pick up the misplaced items and place them in the appropriate bins before checkout. For instance, you will be asked to place socks in a laundry hamper, books in a bookshelf, dishes in a dish bin, etc... You will be performing the task in a 3D virtual environment using keyboard controls, described later.
\end{quote}

The participant is then placed in a virtual environment within the AR simulator described in Sec.\ \ref{sec:arsimulator} and must complete the task using the keyboard navigation and pick/place actions; they can leverage any AR assistance we provide in the HUD. We consider six semantic object categories and employ a specific bin for each category: dishes (dish bin), toys (toy box), books (bookshelf), laundry (laundry hamper), office supplies (office-supply box), recycling (recycling bin). Fig.~\ref{fig:teaser}(a) illustrates some of the objects and bins used in the study. We note that this formulation leads to a capacitated vehicle routing problem as described in Sec.\ \ref{sec:CVRP}, where $\nobjects$ denotes the number objects to be cleaned up, and delivery locations are repeated when more than one object is associated with the same bin. Appendix \ref{sec:houseGeneration} describes how the bins, objects, and starting location are determined for a given experiment.

\subsection{Study conditions: assistance fidelity and task difficulty}\label{sec:studyConditions}

We vary two key variables across experiments: \textit{assistance fidelity}, which represents how much assistance the AR simulator provides to the user toward efficient task completion; and \textit{task difficulty} as measured by the number of objects that must be cleaned up. We hypothesize that these two variables will be the key drivers of the user experience and task performance. We now describe in more detail how we control these variables.

\subsubsection{Assistance Fidelity}

We consider three different levels of assistance fidelity: no assistance, object-highlighting assistance, and optimal assistance. Each assistance level is characterized by both a world-locked digital-object component and a text-information component; see Fig.~\ref{fig:assistance_levels}. In all conditions, text-information assistance includes a list of bins including their picture and semantic location. 


   \textit{No assistance (None)}. Participants receive no assistance from the system in this condition, which serves as our control. The egocentric frame contains only the scene, rendered objects and rendered bins; there are no additional visual cues. The text-information assistance provides a (randomized) list of objects the participant must reorganize in order to complete the task. Each item in this list contains the name of the object, a picture of the object, and the bin in which it should be placed. Once a participant picks up an item, the text corresponding to the selected item is crossed out and move to the bottom of the list.
   
\textit{Object-highlighting assistance}. This form of assistance is designed to provide assistance to the participant under the assumption that the AR device knows the location of the objects and bins salient to the house-cleaning task and can highlight them. Such assistance---which does not rely on knowledge of traversable paths in the environment nor a real-time planner---would be especially helpful in situations where certain items are obstructed from view or are difficult to spot. This form of assistance enables participants to understand the rough locations of all objects at once and form a plan themselves. We implement this form of assistance by placing a digital flagpole over each object as depicted in Fig.~\ref{fig:assistance_levels}; the corresponding text-information assistance includes all of the information from the No-assistance condition but with the addition of the name of the room in which the object can be found. Again, this list is randomized per participant and list items are crossed off as they are completed. 
    
    \textit{Optimal assistance}. Optimal assistance corresponds to the form of AR assistance proposed in Sec.\ \ref{sec:arassistance}. A solution to this problem for the lowest difficulty setting is shown in Fig.~\ref{fig:optimal_solution}. 
    To display this information to the participant, we display the next segment of the optimal path in the egocentric frame as a trail of digital breadcrumbs, which we set to red spheres. After the user executes a feasible pick/place action, we display the next segment of the optimal path (which may involve replanning as described in Sec.\ \ref{sec:arassistance}. To prevent the participant from losing their orientation with respect to these start and end positions of the optimal path segment, the $z$-coordinate of the path's breadcrumbs start at the participant’s chest level and end at the floor level (see Fig.~\ref{fig:assistance_levels}). In contrast to other assistance conditions, the text-information assistance is now ordered according to the optimal path: each step lists the action the participant should take, the object they should perform it on, a picture of this object, and the object’s location. Additionally, each step is numbered in order to emphasize the importance of the list’s order. As before, items are crossed off the list as they are completed.

    %As we are interested in studying this problem in as realistic of a setting as possible, we do not enforce participants to take the precise path that we suggest. This implies that if a participant deviates from the suggested plan, the assistance could become out of step with the plan that the participant is actually executing. As such, we allow the assistance to replan when it determines that the participant has chosen an action that is not in accordance with the provided plan. This is seamless from the participant’s perspective; once they deviate from the provided plan, their actual plan is sent back to our server, where we recalculate the optimal plan given the participant’s current state. This next best plan is then used to provide all future assistance, until replanning is again necessary.



% \textbf{No Assistance}
% Participants receive minimal assistance from the system in this condition, which serves as our control. The egocentric frame contains only the scene, rendered objects and rendered bins; there are no additional visual cues to aid the participant in completing the reorganization task. The text assistance provides a list of objects the participant must reorganize in order to complete the task. Each item in this list contains the name of the object, a picture of the object, and the bin in which it should be placed. This order list is randomized for each participant in order to control for any ordering effects that may be introduced by the list. Once a participant picks up an item, a picture of it is placed into their inventory and the text of the list item is crossed-out and move to the bottom of the list.

% \textbf{Object-highlighting Assistance}
% The object-highlighting assistance is designed to provide assistance to the participant under the assumption that the entire environment (including objects and bins) was scanned. In an AR system, this would allow us to know the precise locations of the objects that need to be reorganized and highlight these in some way so that these locations become obvious to the participant. This would be especially helpful in situations where certain items are obstructed from view or are difficult to spot. Additionally, this assistance level allows a participant to see all of the items at once, and form a plan to complete the task given the location of all of the objects. For our experiment, we highlight the location of the objects by placing a flagpole over each object. This can be seen in the egocentric frame of Figure \ref{fig:assistance_levels}. The text assistance contains all of the information from the No Assistance condition but now additionally includes the name of the room in which the object can be found. Again, this list is randomized per participant and list items are crossed off as they are completed. 

% \textbf{Optimal Assistance} The optimal assistance condition is designed to give participants a complete, optimal solution to the reorganization problem. To obtain this assistance, we again assume that the entire environment is fully scanned. Given this assumption, we can formulate the house reorganization as a vehicle routing problem under the constraints that the participant can hold only two items at a time and that objects must be visited before their respective bins. Additionally, the Habitat simulator allows us to calculate the geodesic distance between all objects in the scene, giving us a cost function we can use to compute a solution to the VRP. Given all of this information, we can generate a provable optimal ordering that would result in the minimum distance travelled to reorganize the house. Furthermore, we can use the Habitat simulator to compute the shortest length trajectory between any two points in the environment. Using these two pieces of information, we can provide the participant with provable optimal assistance both in terms of the order in which they should pick up and place items, as well as the paths they should take to get there. A solution to this problem for the lowest difficulty setting is shown in Figure \ref{fig:optimal_solution}. 

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.85\textwidth]{figs/taskfiles.pdf}
    \caption{The four task-difficulty levels (increasing in difficulty going from left to right), with the optimal path (corresponding to the solution of the associated CVRP) shown in the leftmost panel. Colored polygons represent approximate bounding boxes of the apartment's floor plan, including the boundaries for each rooms; circular markers denote objects; square markers denote bins; marker color denotes semantic object category (e.g., books); the star represents the initial position.}
    \label{fig:optimal_solution}
\end{figure*}

% To display this information to the participant, we can display a single segment of the path in the egocentric frame as a trail of “breadcrumbs”. For these breadcrumbs, we large red spheres. These trails are updated after each time the participant picks or places an object in the environment. The trails start at the participants initial location (when they performed the pick or place action) and end at the location of the next pick or place action they should perform. To prevent the participant from losing their orientation with respect to these start and end positions, the z-axis of the path starts at the participant’s chest level and ends at the floor level. A small segment of this  path can be seen in egocentric frame of Figure \ref{fig:assistance_levels}. The text information is now order dependent and displays exact steps that the participant could take in order to complete the task. Each step contains the action they should perform, the object they should perform it on, a picture of this object, and the object’s location. Additionally each step is numbered in order to indicate that the list’s order matters. As before, items are crossed off as they are completed, however, the lists are no longer randomized. 

% As we are interested in studying this problem in as realistic an environment as possible, we do not enforce that participants take the path that we suggest to them. This means that if a participant deviates from our suggested plan, the assistance could become out of step with the plan that the participant is actually executing. As such, we allow the assistance to replan when it determines that the participant has chosen an action that is not in accordance with the provided plan. This is seamless from the participant’s perspective; once they deviate from the provided plan, their actual plan is sent back to our server, where we recalculate the optimal plan given the participant’s current state. This next best plan is then used to provide all future assistance, until replanning is again necessary. 

\subsubsection{Task Difficulty}

We consider four levels of task difficulty, where we define difficulty in terms of the number of misplaced objects that must be cleaned up. To control for certain objects being easier to reorganize (due to visual salience or bin location), the number of each object type remained fixed for each difficulty setting. A single difficulty level can thus be defined by the ratio of the number of objects to the number of bins. We use four task-difficulty levels, where this ratio corresponds to 1:1 (6 total objects), 2:1 (12 total objects), 3:1 (18 total objects), and 4:1 (24 total objects), respectively. 
Appendix \ref{sec:houseGeneration} describes our approach for generating the bin, object, and initial user locations for any of these conditions.
 Fig.~\ref{fig:optimal_solution} shows the bin locations as squares in each difficulty setting, with each color representing a specific semantic object category. 


\subsection{Metrics}\label{sec:metrics} To determine the effect of assistance fidelity and task difficulty on participants' task performance and experience, we collect an array of objective and subjective participant-response data.

\subsubsection{Objective metrics}
We employ four metrics to evaluate task performance:~(1)~\textit{Normalized Deviations}: the number of deviations from the optimal location ordering (accounting for replanning) normalized by the total number of possible deviations,~(2)~\textit{Inverse Path Length (IPL)}: the ratio of the minimal possible path length for to the sequence of location visits taken by the participant\footnote{That is, $\sum_{i=1}^{2n}\distance{\stepToLocTaken{i}}{\stepToLocTaken{i-1}}$ in the notation of Sec.\ \ref{sec:CVRP}.} to the total distance traveled by the participant,~(3)~\textit{Task Distance}: the total distance traveled by the participant, and~(4)~\textit{Task Completion Time}: the ratio of the total time taken by a participant to complete the task to the time taken by a participant to complete the fly-through familiarization phase; this ratio accounts for any system-dependent latency that may affect completion time.

\subsubsection{Subjective metrics}\label{sec:subjective}
We employ subjective metrics that are measured using a five-point Likert scale, which focus on the following two categories\footnote{These questions only comprise a subset of the questions that we asked in the original study. We limit our analysis here to this subset due to space constraints; see the Appendix~\ref{sec:fullsubjective} for the full list.}:

\begin{enumerate}
    \item \textit{Agency}, which is defined as the feeling of being in control~\cite{moore2016sense}.
    \begin{itemize}
        \item[] ``I am in charge of deciding what step I complete next during the house cleaning task'' (\textit{Control what to do})
        %\item[]``I am in charge of deciding where I go next during the house cleaning task''
        \item[]``I am responsible for the speed at which I completed the task'' (\textit{Control of speed})
        \item[]``I feel that I need to follow the suggestions given to me by the system'' (\textit{Need to follow})
        \item[] ``I prefer that the system show me what to do next rather than figure it out myself during the house cleaning task'' (\textit{Prefer to show})
        %\item[] ``I prefer that the system show me where to go next rather than figure it out myself during the house cleaning task''
    \end{itemize}
    \item \textit{Utility and Usability}, which is aimed at measuring usefulness, user-friendliness, and acceptability; it is inspired by the System Usability Scale (SUS)~\cite{bangor2008empirical}.
    \begin{itemize}
        %\item[] ``I found the house cleaning task more difficult to complete than the training task''
        %\item[] ``I thought the system was easy to use'',
        %\item[]``I would imagine that most people would learn to use the help provided by the system very quickly''
        %\item[]``I would like to use the help provided to me by system during the house cleaning task frequently in real life house cleaning scenarios''
        \item[]``The assistance provided to me by the system during the house cleaning task helped me complete the task faster than if I had used the help provided to me during the training task'' (\textit{Usable})
        \item[] ``I found the help given to me by the system to be useful'' (\textit{Useful})
        %\item[]``The help provided to me by the system during the house cleaning task was sufficient in order to accomplish the task''.
    \end{itemize}
\end{enumerate}




\subsection{HIT overview}\label{sec:hitoverview}



%For a complete breakdown of how many participants were in each condition, see Table \ref{tab:participants}.

%\begin{figure*}[ht]
%    \centering
%    \includegraphics[width=0.95\textwidth]{figs/kondo_phases.png}
%    \caption{The five phases of our experiment. Phases 1 through 3 are used to familiarize participants to the task. Phase 4 is the experimental phase, where participants are randomly split into one of the 12 different conditions. Finally, participants are taken to the final phase: the post-experiment survey.}
%    \label{fig:trial_timeline}
%\end{figure*}

The HIT for the study consists of four phases:~(1)~task setup,~(2)~house familiarization and navigation-controls training,~(3)~cleaning-task execution, and~(4)~survey. In the first phase, the participant is presented with the house-cleaning-scenario prompt described in Sec.\ \ref{sec:task}. In the second phase, the participant is familiarized with the 3D layout of the short-term rental house using a pre-recorded fly-through video that displays information regarding room names and bins locations. To acquaint the participant with the keyboard controls, they are given a simple training task of finding and picking up a single object and placing it in its appropriate bin without any imposed time limit or incentive. The third phase corresponds to executing the main cleaning task described in Sec.\ \ref{sec:task} with specified task-difficulty and assistance-fidelity levels. In the final phase, the participant is given a survey that collects demographic information (e.g., age, gender), responses to the subjective questions described in Sec.\ \ref{sec:subjective}, and a free-form response to capture anything else relevant to their experience. Except for the actual task in the third phase of the HIT---which varied across participants depending on the study conditions described in Sec.\ \ref{sec:studyConditions}---all other phases were consistent across participants.

% In the first phase, participants were given general instructions about the experiment. This included information about these phases, compensation amount, estimated task completion time, any known technical difficulties, and information on how to contact us if something went wrong while completing the experiment. Participants were additionally introduced to the main purpose of the task through the following paragraph: 

% This prompt was designed to situate participants to the task and add a small amount of urgency to the task completion. Participants were not actually “charged a fee” in either real or virtual currency.  The second phase of the study was designed to familiarize participants with the layout of the 3D apartment rendering. A single apartment layout (consisting of the 3D rendering and bin placements) was used for every condition. In this phase, the user was shown a prerecorded video of an agent walking through the 3D environment. The agent paused whenever it entered a new room or got close to one of the bins. In addition to the egocentric rendering of the environment, the participant was shown a short message placed above the video frame with a phrase telling the user what room they currently occupied and if any bins were place in that room. 

% The third phase was designed to familiarize participants with the navigation controls. Participants could navigate through the environment by rotating the egocentric frame either left or right (by using the arrow keys) or by moving forward (by pressing the w key). Additionally, participants could pick and place objects by pressing the spacebar. To familiarize participants with this control scheme, they were task with a simple task to complete in the environment: find a single object, pick it up, and place it in the appropriate bin. Each participant saw the same training task and there was no limit on the amount of time they could spend in the training task. 

% The fourth phase of the experiment was the task. At this point, the experiment branched into three categories based on the assistance condition assigned at the beginning of the HIT. In each branch, participants were first shown a set of instructions that were unique to the assistance condition they were assigned. Once they finished reading these instructions, they advanced to complete the house cleaning task. The specific house cleaning task that was displayed to the user depended on the task difficulty that was assigned at the beginning of the HIT. Once the participant placed the final object, they were automatically advanced to the final phase.

% The fifth and final phase of the study consisted of the post-experiment survey. In this survey, we collected demographic information (\textit{e.g.}, age and gender) as well as subjective responses to questions about the task. All subject questions were asked on a 5-point scale: Strongly Disagree, Disagree, Neutral, Agree, Strongly Agree. Following the subjective response questions, participants were given an opportunity for free response. Each participant saw the same survey. Participants needed to complete all survey questions in order to complete the HIT and have their data be recorded. 



==> Kondo Public/systemoverview.tex <==
\subsection{System overview}
Our Human Intelligence Task (HIT) was served to Amazon Mechanical Turk (AMT) \cite{} using a psiturk \cite{} server, and allowed us to advertise our HIT on through the AMT web portal. Through this portal, they could see a short description of the study, compensation, and the estimated completion time. Once they accepted our HIT on AMT, they were taken through a consent procedure. After accepting to participate in our study, the Habitat WebGL application \cite{} was served to the user’s web browser using a combination of a psiturk server and an nginx server \cite{}. At this time, the participant’s condition was randomly sampled from both independent variables (i.e. assistance condition and task difficulty). The majority of the application was loaded directly onto the participant’s computer, with the exception of the replanning module. When a disagreement between the participant’s actual path and our calculated optimal path occured (as measured by the participant interacting with a different object than the one we calculated to be optimal through the VRP Solver), the participant’s web browser communicated with the psiturk server and recalculated the optimal path given the participant’s current completed path. After completing the survey, the data collected during the experiment (e.g. keyboard actions, time spent completing each phase, survey responses, number of recalculations, new paths resulting from calculations, inventory status, etc…) was transmitted back to our server where it was stored in a MySQL database \cite{} for later use. After the participant completed the experiment, the researchers used psiturk to approve and disburse payment through AMT. If any issues arose during the completion of the experiment, participants were provided with a code they could use to redeem payment for their participation through a separate psiturk experiment WhoopsY’all \cite{} This setup allowed us to have many participants completing our task in parallel, but did put a burden on the participants computing ecosystem to be able to load and run the ~8Gb WebGL application. 


==> systemoverview.tex <==
\subsection{System overview}
Our Human Intelligence Task (HIT) was served to Amazon Mechanical Turk (AMT) \cite{} using a psiturk \cite{} server, and allowed us to advertise our HIT on through the AMT web portal. Through this portal, they could see a short description of the study, compensation, and the estimated completion time. Once they accepted our HIT on AMT, they were taken through a consent procedure. After accepting to participate in our study, the Habitat WebGL application \cite{} was served to the user’s web browser using a combination of a psiturk server and an nginx server \cite{}. At this time, the participant’s condition was randomly sampled from both independent variables (i.e. assistance condition and task difficulty). The majority of the application was loaded directly onto the participant’s computer, with the exception of the replanning module. When a disagreement between the participant’s actual path and our calculated optimal path occured (as measured by the participant interacting with a different object than the one we calculated to be optimal through the VRP Solver), the participant’s web browser communicated with the psiturk server and recalculated the optimal path given the participant’s current completed path. After completing the survey, the data collected during the experiment (e.g. keyboard actions, time spent completing each phase, survey responses, number of recalculations, new paths resulting from calculations, inventory status, etc…) was transmitted back to our server where it was stored in a MySQL database \cite{} for later use. After the participant completed the experiment, the researchers used psiturk to approve and disburse payment through AMT. If any issues arose during the completion of the experiment, participants were provided with a code they could use to redeem payment for their participation through a separate psiturk experiment WhoopsY’all \cite{} This setup allowed us to have many participants completing our task in parallel, but did put a burden on the participants computing ecosystem to be able to load and run the ~8Gb WebGL application. 

